Categorical Foundations of Explainable AI: A Unifying Theory

Explainable AI (XAI) aims to address the human need for safe and reliable AI systems. However, numerous surveys emphasize the absence of a sound mathematical formalization of key XAI notions -- remarkably including the term "explanation" which still lacks a precise definition. To bridge this gap, this paper presents the first mathematically rigorous definitions of key XAI notions and processes, using the well-funded formalism of Category theory. We show that our categorical framework allows to: (i) model existing learning schemes and architectures, (ii) formally define the term "explanation", (iii) establish a theoretical basis for XAI taxonomies, and (iv) analyze commonly overlooked aspects of explaining methods. As a consequence, our categorical framework promotes the ethical and secure deployment of AI technologies as it represents a significant step towards a sound theoretical foundation of explainable AI.

==> todo_last.tex <==
-) citazioni pre 4.3, 2 so già dette nell'intro.. metterne altre? 

-) che significano esattamente: "In fact, our definition of explanation can provide (i) additional meta information to describe properties related to the explainer, or (ii)  the feature relevance of an input, or (iii) an answer to why an input instance leads to a specific output."

-) Backward-based explainer: nabla e la loss so sempre sganciati, ho messo frase in generale.. basta?

-) "The following examples show the relation between a syntactic and a semantic techniques emphasizing connections between XAI methods that often slip unnoticed."
Questa mi pare un po' troppo! vediamo se almeno si mette un esempio senzato ahahahah

-) es. 4.5 da decidere se sono solo alcuni modelli e l'istituzione è semplicemente FO1 (cioè FOL con un solo predicato nelle signatures)

-) "For this reason, a promising but often overlooked research direction consists in accurately lifting semantic explanations into a symbolic language in order to provide a syntactic explanation~" si menziona studi di modelli trasparenti? problema spesso riducono performances..., ma c'è qualcosa che si muove di novo.. E-LEN, DCR..

-) "As with any mathematical theory, our approach represents one of the possible formalizations of foundational notions of XAI." 
DA LEVARE ASSOLUTAMENTE! (mmm in parte va detto, magari riformulare)

-) "Cartesian streams form a feedback cartesian monoidal category, i.e are equipped,80
for every object X, with morphisms νX : X → X × X and εX : X → e that allow to copy and81
discard objects (cf. Appendix A.2). This makes them the ideal category to formalize (possibly82
infinite) streams of objects and morphisms.83" Mi sembra molto debole dire solo "oh bada l'ha fatto Katsumata allora". La sensatezza della scelta stava nella descrizione del feedback ecc.

IMPORTANTE!!!
mettere silency a k pixel e FI a m features come 2 signature diverse all'interno del FOL fragment
 

